An $\alpha$-No-Regret Algorithm For Graphical Bilinear Bandits

We propose the first regret-based approach to the Graphical Bilinear Bandits problem, where $n$ agents in a graph play a stochastic bilinear bandit game with each of their neighbors. This setting reveals a combinatorial NP-hard problem that prevents the use of any existing regret-based algorithm in the (bi-)linear bandit literature. In this paper, we fill this gap and present the first regret-based algorithm for graphical bilinear bandits using the principle of optimism in the face of uncertainty. Theoretical analysis of this new method yields an upper bound of $\tilde{O}(\sqrt{T})$ on the $\alpha$-regret and evidences the impact of the graph structure on the rate of convergence. Finally, we show through various experiments the validity of our approach.

==> related.tex <==
\section{Related Work}
\label{sec:related_work}

The Graphical Bilinear Bandit setting has been first established in \citet{rizk2021best} where they tackle the problem of identifying the $1/2$-best joint arm (which has an associated reward equal to at least $1/2$ of the optimal one). They choose a pure exploration approach and give an algorithm that choose at each round the arms that follows a G-allocation strategy. They do not intend to maximise the cumulative reward (or equivalently minimize the associated regret) and thus they do not deal with the trade-off between exploration and exploitation. We fill this gap in this paper and propose two first regret-based algorithms for the Graphical Bilinear Bandits setting. 

Other works tackle bandit problems in graph. On one hand, in \citep{valko2014spectralbandits,mannor2011bandits} for instance, they represent a bandit problem through a graph but it is a single agent problem and the nodes of the graph represent arms that, when they are pulled, give information on their neighbouring arms. On the other hand, in \citet{cesa2013gang} each node is an instance of a linear bandit and the neighboring nodes are assumed to have similar unknown regression coefficients. The main difference with our setting is that the rewards of the nodes are independent.
\geovani{Derniere phrase a reformuler: mot pour mot celle qu'on a mise dans le papier ICML}

\geovani{Paragraphe sur bandit lineaire en parallele}

\geovani{Paragraphe sur combinatorial bandits. Expliquer que c'est dans cette literature que le $\alpha$-regret a été utilisé, car on traite des problèmes NP-Hard.}

\textbf{Combinatorial and multi-agent bandits.} Allocating arms to each node of a graph to then observe a global reward is a combinatorial bandit problem \citep{cesabianchi2012}, the number of joint arms scaling exponentially with the number of nodes. This has been studied in the regret-based context \citep{chen2013combinatorial,Perrault2020} and more particularly in \citet{qin2014contextual} where the reward associated to each arm is linear (each arm having a vector representation). Our problem can fit into the setting of this last cited paper but with two condition: the agents must be centralized and one has to have access to an Oracle to solve the combinatorial optimization problem returning the arm to play each turn. We make no such assumption on the existence of the oracle.
Finally, most of the algorithms developed for combinatorial bandits assume the availability of an oracle to solve the combinatorial optimization problem returning the arm to play. We make no such assumption.



